Beyond Self-Similarity: Reconciling X-Ray Scaling Relations in Galaxy Clusters and Groups

Scaling relations hold among observed quantities that describe the thermodynamic properties of the gas in galaxy clusters and groups. However, observed data show systematic departures from the self-similar model's baseline predictions, particularly in lower-mass systems. I show that the observed departures from self-similar predictions can be efficiently described by two physical quantities modeled with power laws: the gas mass fraction $f_g$ and the temperature variation $f_T$. Using a wide range of published X-ray scaling relations, this study conducts an MCMC-based meta-analysis to constrain the temperature- and redshift-dependence of the meta-parameters $f_g$ and $f_T$ and calibrate the model. These calibrations indicate that, while the gas mass fraction does not show significant evolution with cosmic time, it decreases significantly with decreasing halo mass. On the other hand, the temperature variation shows a mild positive increase with both mass and redshift. Overall, modeling the departures from the self-similar model with $\{f_g, f_T\}$ drastically improves predictive accuracy, reducing the number of scaling relations in $>3\sigma$ ($>5 \sigma$) tension from 49 (36) percent under the self-similar scenario to just 8 (3) percent (three and one out of 39, respectively) that might be identified for their peculiarity. Moreover, modeling through this generalized framework allows for an extended discussion of the expected slopes and redshift evolution for several X-ray scaling laws, including the new quantity $Y_{LGT0} = L^{-1} M_g^2 T^{a_L}$, a proxy for the cluster's volume that is independent of $f_g$ and $f_T$ by construction, and is predicted to scale directly with mass with a well-defined redshift evolution ($M \sim Y_{LGT0} f_g^0 f_T^0 E_z^2$), as validated against hydrodynamical simulations and observational constraints.

==> figures/relations.tex <==
\setlength\tabcolsep{2.2pt} \begin{center} \begin{tabular}{cccccc} \hline
Ref. & Par. & value & $N_{\rm obj}$ & $\Delta M$ ($10^{14} M_{\odot}$) & $\Delta z$ \\ \hline
R11 & $B_{LbT}$ & $2.70 \pm 0.24$ & 232 & 0.5 - 20.0 & 0.30 - 1.46 \\
R11 & $C_{LbT}$ & $-0.23 \pm 0.37$ &  -  &  -  &  -  \\
R11 & $B_{LbM}$ & $1.92 \pm 0.11$ &  -  &  -  &  -  \\
R11 & $C_{LbM}$ & $1.73 \pm 0.49$ &  -  &  -  &  -  \\
S20 & $B_{L5M}$ & $1.06 \pm 0.35$ & 105 & 0.1 - 10.0 & 0.05 - 1.10 \\
S20 & $C_{L5M}$ & $2.10 \pm 2.08$ &  -  &  -  &  -  \\
S20 & $B_{MT}$ & $1.18 \pm 0.43$ &  -  &  -  &  -  \\
S20 & $C_{MT}$ & $-0.21 \pm 0.78$ &  -  &  -  &  -  \\
L20 & $B_{L1M}$ & $1.67 \pm 0.18$ & 120 & 2.4 - 17.6 & 0.06 - 0.55 \\
L20 & $C_{L1M}$ & $1.33 \pm 0.80$ &  -  &  -  &  -  \\
L20 & $B_{L1T}$ & $2.41 \pm 0.29$ &  -  &  -  &  -  \\
L20 & $C_{L1T}$ & $1.17 \pm 0.82$ &  -  &  -  &  -  \\
L20 & $B_{MYx}$ & $0.54 \pm 0.03$ &  -  &  -  &  -  \\
L20 & $C_{MYx}$ & $-0.29 \pm 0.29$ &  -  &  -  &  -  \\
L21 & $B_{L1T}$ & $2.48 \pm 0.04$ & 40 & 0.1 - 10.0 & 0.01 - 0.80 \\
L21 & $B_{MT}$ & $1.76 \pm 0.02$ &  -  &  -  &  -  \\
L21 & $B_{L1M}$ & $1.42 \pm 0.03$ &  -  &  -  &  -  \\
B22 & $B_{L5T}$ & $2.89 \pm 0.14$ & 265 & 0.1 - 7.8 & 0.02 - 0.94 \\
B22 & $C_{L5T}$ & $1.59 \pm 0.90$ &  -  &  -  &  -  \\
B22 & $B_{L5Mg}$ & $1.10 \pm 0.03$ &  -  &  -  &  -  \\
B22 & $C_{L5Mg}$ & $1.44 \pm 0.26$ &  -  &  -  &  -  \\
P22 & $B_{LbM}$ & $1.74 \pm 0.02$ & 93 & 0.5 - 20.0 & 0.05 - 1.13 \\
P22 & $C_{LbM}$ & $2.50 \pm 0.09$ &  -  &  -  &  -  \\
P22 & $B_{LbYx}$ & $0.97 \pm 0.02$ &  -  &  -  &  -  \\
P22 & $C_{LbYx}$ & $1.79 \pm 0.08$ &  -  &  -  &  -  \\
P25 & $B_{L5M}$ & $1.47 \pm 0.03$ & -1 & 0.1 - 1.0 & 0.00 - 0.20 \\
T25 & $B_{MT}$ & $1.65 \pm 0.11$ & -1 & 0.1 - 5.0 & 0.00 - 0.20 \\
R26 & $B_{L5T}$ & $2.51 \pm 0.04$ & 3061 & 0.1 - 16.0 & 0.05 - 1.07 \\
R26 & $C_{L5T}$ & $1.88 \pm 0.35$ &  -  &  -  &  -  \\
R26 & $B_{L5Mg}$ & $1.23 \pm 0.01$ &  -  &  -  &  -  \\
R26 & $C_{L5Mg}$ & $2.16 \pm 0.07$ &  -  &  -  &  -  \\
R26 & $B_{MgT}$ & $2.24 \pm 0.03$ &  -  &  -  &  -  \\
R26 & $C_{MgT}$ & $-1.00 \pm 0.30$ &  -  &  -  &  -  \\
E26 & $B_{L5T}$ & $2.54 \pm 0.19$ & 44 & 0.1 - 1.0 & 0.00 - 0.05 \\
M26 & $B_{L5T}$ & $2.90 \pm 0.10$ & 155 & 0.1 - 5.5 & 0.07 - 0.20 \\
O26 & $B_{LbT}$ & $2.09 \pm 0.51$ & 27 & 3.0 - 20.0 & 0.14 - 1.17 \\
O26 & $C_{LbT}$ & $1.89 \pm 1.97$ &  -  &  -  &  -  \\
O26 & $B_{LbM}$ & $1.35 \pm 0.85$ &  -  &  -  &  -  \\
O26 & $C_{LbM}$ & $3.44 \pm 1.50$ &  -  &  -  &  -  \\
\hline \end{tabular} \end{center}


==> figures/relations2.tex <==
\begin{center} \begin{tabular}{ccccc} \hline
$Q_{\Delta}$ & $a_T$ & $a_{T, z}$ & $a_M$ & $a_{M, z}$ \\ \hline
 $T_{\Delta}$ & $1.15 \; (0.01)$ $[1]$ & $0.11 \; (0.07)$ $[0]$ & $2/3$ \; $[2/3]$ & $2/3$ \; $[2/3]$ \\
 $n_{\Delta}$ & $0.50 \; (0.01)$ $[0]$ & $1.89 \; (0.03)$ $[2]$ & $0.29 \; (0.01)$ $[0]$ & $2.13 \; (0.04)$ $[2]$ \\
 $P_{\Delta}$ & $1.65 \; (0.01)$ $[1]$ & $2.01 \; (0.07)$ $[2]$ & $0.96 \; (0.01)$ $[2/3]$ & $2.80 \; (0.04)$ $[8/3]$ \\
 $K_{\Delta}$ & $0.82 \; (0.01)$ $[1]$ & $-1.15 \; (0.07)$ $[-4/3]$ & $0.47 \; (0.01)$ $[2/3]$ & $-0.76 \; (0.04)$ $[-2/3]$ \\
 EM$_{\Delta}$ & $1.57 \; (0.01)$ $[1/2]$ & $2.85 \; (0.07)$ $[3]$ & $0.91 \; (0.01)$ $[1/3]$ & $3.60 \; (0.09)$ $[10/3]$ \\
\hline \end{tabular} \end{center}


==> figures/relations_bf.tex <==
\begin{center} \begin{tabular}{ccc} \hline
 Rel.  &   $B$  &  $C$  \\  \hline
MT & $1.730 \, (0.012) \, [1.500]$ & $-0.829 \, (0.101) \, [-1.000]$ \\
MgT & $2.229 \, (0.014) \, [1.500]$ & $-0.934 \, (0.106) \, [-1.000]$ \\
MYx & $0.536 \, (0.008) \, [0.600]$ & $-0.366 \, (0.047) \, [-0.400]$ \\
LbT & $3.178 \, (0.018) \, [1.950]$ & $0.961 \, (0.120) \, [1.000]$ \\
L1T & $2.597 \, (0.018) \, [1.370]$ & $0.961 \, (0.120) \, [1.000]$ \\
L5T & $2.608 \, (0.120) \, [1.380]$ & $0.961 \, (0.120) \, [1.000]$ \\
LbM & $1.837 \, (0.010) \, [1.300]$ & $2.484 \, (0.107) \, [2.300]$ \\
L1M & $1.502 \, (0.009) \, [0.913]$ & $2.206 \, (0.083) \, [1.913]$ \\
L5M & $1.508 \, (0.009) \, [0.920]$ & $2.211 \, (0.084) \, [1.920]$ \\
LbMg & $1.426 \, (0.003) \, [1.300]$ & $2.293 \, (0.021) \, [2.300]$ \\
L1Mg & $1.166 \, (0.003) \, [0.913]$ & $2.050 \, (0.032) \, [1.913]$ \\
L5Mg & $1.170 \, (0.003) \, [0.920]$ & $2.054 \, (0.032) \, [1.920]$ \\
\hline \end{tabular} \end{center}

